SynFog: A Photo-realistic Synthetic Fog Dataset based on End-to-end Imaging Simulation for Advancing Real-World Defogging in Autonomous Driving

To advance research in learning-based defogging algorithms, various synthetic fog datasets have been developed. However, existing datasets created using the Atmospheric Scattering Model (ASM) or real-time rendering engines often struggle to produce photo-realistic foggy images that accurately mimic the actual imaging process. This limitation hinders the effective generalization of models from synthetic to real data. In this paper, we introduce an end-to-end simulation pipeline designed to generate photo-realistic foggy images. This pipeline comprehensively considers the entire physically-based foggy scene imaging process, closely aligning with real-world image capture methods. Based on this pipeline, we present a new synthetic fog dataset named SynFog, which features both sky light and active lighting conditions, as well as three levels of fog density. Experimental results demonstrate that models trained on SynFog exhibit superior performance in visual perception and detection accuracy compared to others when applied to real-world foggy images.

==> sec/6_discussion.tex <==
\section{Discussion and Limitation}
\label{sec:discussion}
\par \iffalse The proposed end-to-end foggy image simulation pipeline offers a significant advantage by integrating a more precise scattering process modeling, as well as realistic camera processing, particularly through physically-based sensor modeling. This results in noticeable consistency, where the noise level increases as the fog density rises. As a result, models trained on our dataset demonstrate better generalization to real-world data compared to existing synthetic datasets.\fi Experimental results indicate that models trained on SynFog with realistic physical characteristics of optics and sensors demonstrate a more robust performance on real-word fog datasets, both in terms of visual perception and detection accuracy. This finding suggests that incorporating a physically-based end-to-end imaging process replicating real capture methods can significantly enhance the generalization of trained models. However, due to the time-consuming nature of the physically-based volumetric path tracing technique, the scale of SynFog is not as extensive as other synthetic datasets. Nevertheless, we are dedicated to expanding the scene contents in the future and considering a wider range of scattering mediums beyond just fog.

\vspace{-0.3cm}

==> sec/8_acknowledgement.tex <==
\section{Acknowledgement}
\label{sec:acknowledgement}
\par We thank Professor Chuxi Yang and Jiayue Xie for their help in preparing the scene creation. We also thank Professor Brian Wandell, Dr. Devesh Upadhyay, Dr. Alireza Rahimpour, and Devesh Shah for their valuable advice at the early stage of this project.
